Gradient-Free Generation for Hard-Constrained Systems

Generative models that satisfy hard constraints are critical in many scientific and engineering applications, where physical laws or system requirements must be strictly respected. Many existing constrained generative models, especially those developed for computer vision, rely heavily on gradient information, which is often sparse or computationally expensive in some fields, e.g., partial differential equations (PDEs). In this work, we introduce a novel framework for adapting pre-trained, unconstrained flow-matching models to satisfy constraints exactly in a zero-shot manner without requiring expensive gradient computations or fine-tuning. Our framework, ECI sampling, alternates between extrapolation (E), correction (C), and interpolation (I) stages during each iterative sampling step of flow matching sampling to ensure accurate integration of constraint information while preserving the validity of the generation. We demonstrate the effectiveness of our approach across various PDE systems, showing that ECI-guided generation strictly adheres to physical constraints and accurately captures complex distribution shifts induced by these constraints. Empirical results demonstrate that our framework consistently outperforms baseline approaches in various zero-shot constrained generation tasks and also achieves competitive results in the regression tasks without additional fine-tuning.

==> secs/STALE_abstract.tex <==
\begin{abstract}
% Recently, machine learning models have been applied to solving partial differential equations (PDEs) as a deterministic operator is learned between function spaces. 
Inspired by the success of generative models in computer vision, generative frameworks for solving partial differential equations (PDEs) have been recently explored. 
However, applications in the PDE domain often require the generated solutions to adhere to certain physical constraints or to satisfy certain boundary conditions. 
The incorporation of such physical constraints during the sampling step of the generative process remains largely unexplored.
% Most existing studies focus on predicting PDE solutions based on input conditions, primarily through regression-based approaches. However, these methods typically necessitate training separate models for each set of constrained conditions.
%Prior work predominantly focused on regression tasks, in which a deterministic operator is learned between function spaces.
%This approach fails to capture the generative characteristics of \emph{underspecified} PDE systems with infinitely many possible solutions due to the lack of constraints or variations in the PDE parameters.
% \michael{Clarify why?}
% With infinitely many possible solutions in underdetermined PDE systems, a generative model is necessary to capture the distributional properties.
% \michael{I don't understand the contrast with the previous sentence; underdetermined is still regression.}
%Although generative models on function spaces have been proposed, the incorporation of physical constraints during the sampling step of the generative process remains underexplored.
A challenge is that existing constrained generative models, particularly from the computer vision domain, typically rely on gradient information, which can be either too sparse or prohibitively expensive to compute for PDE data.
%%To develop a unified framework for handling various constraints, 
To address these challenges, we propose a new unified framework for handling various posterior constraints when generating PDE solutions.
Our approach, which we call \emph{ECI sampling}, consists of interleaved extrapolation (E), correction (C), and interpolation (I) steps in each sampling iteration. 
ECI sampling guides a 
%\michael{What does that word mean?  ``unconstrained''? If so, is there a reason not to use that word to clarify?}
pre-trained unconstrained generative model to the constrained set of solutions in a zero-shot manner, and without the need for expensive fine-tuning or gradient calculations. 
Our ECI sampling effectively facilitates the mixing of information between the constrained and unconstrained regions, while enjoying the exact satisfaction of the constraints.
% \michael{Clarify that that is at each step, not necessarily the final solution.}
%Our approach provides a unified framework for different constraints and is optimization-free without expensive fine-tuning or gradient calculations. 
% \michael{We need to be more precise throughout;  we are using the word ``constraints'' in a different way that e.g. Derek did.}
Empirical results on various PDE systems demonstrate that our ECI-guided generation can accurately capture the distribution shift imposed by the constraints, when compared to other baselines. 
In addition, when tested in zero-shot regression scenarios, our method continues to outperform existing approaches.%  while maintaining the physical consistency of the PDE system. 
% In addition, ECI also achieves competitive performance on zero-shot regression tasks with traditional neural operators directly trained on regression objectives.
\end{abstract}


==> secs/STALE_introduction.tex <==
\section{Introduction}

Partial differential equations (PDEs) are fundamental tools in various scientific domains, from fluid dynamics and heat transfer to electromagnetism and quantum mechanics. 
Machine learning (ML) models have advanced in solving PDE systems, as a learnable mapping between function spaces, obtaining significant speedup and good accuracy. 
These models, known as neural operators (NOs) \citep{lu2019deeponet,li2020neural,li2020fourier,kovachki2023neural}, learn a deterministic mapping between function spaces such that for well-posed PDE systems, the solution exists and is uniquely determined by the input function. 
% \michael{That's not quite the definition of well-posed; is that what we are referring to here? That word is used in the next sentence.}
%While working with well-posed PDE systems is common, we note the ubiquity of \emph{underspecified} PDE systems in many real-world scenarios.
With the remarkable success of the generative frameworks of diffusion and flow matching in the image generation domain, recent attempts have been made to adopt such frameworks as the generative approaches for finding solutions for underspecified PDE systems with infinitely many solutions. 
In particular, Functional Flow Matching (FFM) \citep{kerrigan2023functional} recently extended the conditional flow matching (CFM) \citep{lipman2022flow} framework for image generation to function spaces for capturing the target measure over a family of continuous functions.

Despite the success of existing models, we noted that applications in the PDE domain often require the generated solutions to adhere to certain physical constraints or to satisfy certain boundary conditions. While such a constrained prediction for regression models has been explored \citep{saad2022guiding,negiar2022learning,li2024physics}, the incorporation of such constraints during the iterative sampling process of generative models remains largely unexplored.
% This inefficient approach poses a significant challenge in practical scenarios where constraints like BC or IC may change.
% To overcome this inefficiency, we aim to develop a general framework that can accommodate infinitely many possible solutions, allowing constraints to be applied during inference without being specified during the pre-training stage.
%In these cases, due to variations in the PDE parameters or the lack of enough initial condition (IC) or boundary condition (BC), the solutions are non-unique \citep{cardiff2008efficient,meng2014lsrn,assous2014indeterminate}. 
% \michael{This is confusing and non-standard.  Perhaps we should use the term "underspecified" or something like that; underdetermined really has a precise meaning in PDE-land, and we are not using it that way.  (I'm not familiar with 2302.12904, and if they have a generalized definition that plays better with ML and is consistent with the usual definition, we should definitely spend the space to explain that.)}
%underspecified PDE systems that have infinitely many possible solutions are less explored in Scientific ML (SciML), and 
% One approach to learning a family of solutions is to leverage generative models during unconditional pretraining, rather than relying on a single deterministic mapping. 
Furthermore, as more constraints are imposed, the set of possible solutions also narrows accordingly. Given these considerations, our proposed framework needs to enable zero-shot constrained generation in unconstrained pre-trained models to capture the distribution shift when various constraints are applied. 

Although it is always possible to train a conditional generative model on such constraints \citep{kerrigan2023functional}, it requires training separate models for each different family of constraints for optimal performance. 
Although prior work has explored the use of diffusion models and FFM for SciML \boran{can you cite papers here}, most studies focus on training conditional generative models. Such training requires prior knowledge of the family of constraints and cannot provide a unified framework that transfers easily between different families of constraints in a zero-shot manner. Therefore, it remains underexplored how to incorporate posterior constraints during sampling, particularly in a zero-shot fashion.
%Although it is always possible to train a conditional generative model, such training requires prior knowledge of the family of constraints and cannot provide a unified framework that easily transfers between different families of constraints in a zero-shot manner.

Unlike controlled generation in the more well-explored computer vision (CV) domain, constrained generation for 
complex dynamical %%underspecified PDE 
systems poses different challenges. 
Specifically, constraints in PDE systems can be much sparser. 
% \michael{What does ``sparser'' mean? Fewer? Or more zeros in each?}
% \michael{@chaoran: I see my comments are commented out, with comments from you on the side.  More important than answering my comments on the side box is that my questions are clarified in the text for the reader. Perhaps you did that for this and other comments, but please be sure to do so.}
Unlike tasks such as image inpainting which usually assumes a considerable amount of context information, constraints like boundary and initial conditions for a PDE system have measure zero in the spatiotemporal domain. 
% \michael{Somewhere, we should say something about how failure to respect hard constraints hardly leads to various failure modes.}
For example, when the IC is prescribed as the constraint, a spatiotemporal size resolution of $100 \times 100$ leads to only 1\% of known pixel values as the context.
% \michael{That sentence is a statement about what we do, not why PDE systems are naturally sparse; can we modify.}
Furthermore, some constraints in PDE systems have strong physical meaning (e.g., conservation laws of mass, energy, or momentum). 
As a result, it is generally expected that these constraints should be satisfied exactly to ensure a physically feasible and consistent solution.
In contrast, for inverse problems in CV, such as super-resolution and de-blurring, constraints are often implicitly defined and need not hold exactly. The evaluation metrics such as the peak signal-to-noise ratio (PSNR) also do not directly depend on the exact satisfaction of those constraints.
Furthermore, existing zero-shot frameworks for constrained image generation predominantly rely on gradient guidance from some differentiable cost function on the last step of generation. 
% \michael{Huh?  What does that sentence mean?  Is ``gradient guidance'' the usual Lagrange dual things?  And how does that relate to zero-shot, since it is more general?}
Of course, such an approach can always be adapted in PDE scenarios; but it does not guarantee the exact satisfaction of the constraints (which is known to lead to ``failure modes'' in other SciML tasks~\citep{krishnapriyan2021characterizing}), and it can be prohibitively expensive for large 3D spatiotemporal PDE systems.
\michael{The sparsity issues probably applies to supply chain use cases also.  I'm sure that the gradient issues also applies.}

\michael{I'm still trying to figure out what are the key issues where vanilla CV methods won't work. One is the sparsity issue. Another is the gradient guidance issue. What else?  And how broad a range of applications do we think those apply? (PDEs, supply chain, what else?) Some of the text is written as if continuous functions versus not is the key issue.  It sounds like this paper has a niche if we can say that those issues are important and that we solve it.}

To address the unique challenges of constrained generation in the PDE domain, we propose a general pipeline to guide an FFM pre-trained on PDE solutions, using zero-shot and gradient-free guidance for constrained generation. 
\michael{Are these challenges unique to PDEs?  Or to any area that needs hard constraints satisfied? Also, are we training a model, or is the FFM pre-trained? See side comments.}
By interleaving \emph{extrapolation}, \emph{correction}, and \emph{interpolation} (for which we termed \emph{ECI}) at each iterative sampling step, our sampling scheme effectively facilitates the mixing of information between the constrained and unconstrained regions.
For diverse practical constraints, ranging from BC and IC to conservation laws of physical quantities, our proposed framework provides a unified and efficient framework that ensures the exact satisfaction of the constraints, without the need for expensive finetuning or gradient backpropagation. 
\michael{But we don't conserve the conserved quantity on the final solution, do we? See side comments.}
Extensive experiments across various PDE datasets demonstrate that our ECI scheme can accurately capture the distribution shift imposed by the constraints while maintaining the physical consistency of the PDE system. Comprehensive generative metrics of distributional properties manifest the superior generative performance of our ECI framework compared with various existing zero-shot guidance methods. 
In addition, we also demonstrate that our ECI framework for guiding pre-trained generative models can be applied to zero-shot regression tasks, in which the constrained generations still achieve competitive performance with the traditional NOs that are directly trained on the regression tasks.

\michael{What step of ECI does the constraint satisfaction hold? I thought it held for the generation step, and then one step undid them, except for special parameter settings.  If we can use this to solve vanilla constrained convex optimization problem, that's different.  So we need to clarify how we are not doing this.}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/model.png}
%     \vspace{-1em}
%     \caption{Overall view of ECI sampling scheme that comprises of multiple interleaved iterations of extrapolation, correction, and interpolation in one Euler step.
%     \michael{This is not a good figure qua figure, in that it does not illustrate the C and I step of ECI; can we come up with something more visually obvious.}
%     }
%     \label{fig:model}
% \end{figure}

% \michael{I like ``system'' and not ``PDE system'' in the title.  But how general is out method, e.g., other dynamical systems, iterative supply chain dynamics, etc}
% \michael{There is discussion in inverse problems; do we evaluate out approach on UQ/inverse problems below.}

==> tabs/ffm_stats.tex <==
\begin{table}[ht]
\centering
\caption{Generative metrics for the prior unconstrained FFM.} \label{tab:ffm_metric}
\vspace{-0.5em}
\begin{tabular}{@{}lcccc@{}}
\toprule
Dataset & MMSE / $10^{-2}$ & SMSE / $10^{-2}$ & CE / $10^{-2}$ & FPD \\ \midrule
Stokes IC & 2.068 & 1.572 & 9.792 & 13.342 \\
Stokes BC & 3.695 & 3.320 & 177.297 & 2.824 \\
Heat Equation & 3.954 & 4.737 & 49.296 & 2.799 \\
Darcy Flow & 58.879 & 69.432 & $7.48\times 10^4$ & 189 \\
NS Equation & 18.749 & 8.423 & 11.451 & 2.185 \\ \bottomrule
\end{tabular}
\end{table}

